Semi-supervised Active Regression

Labelled data often comes at a high cost as it may require recruiting human labelers or running costly experiments. At the same time, in many practical scenarios, one already has access to a partially labelled, potentially biased dataset that can help with the learning task at hand. Motivated by such settings, we formally initiate a study of $semi-supervised$ $active$ $learning$ through the frame of linear regression. In this setting, the learner has access to a dataset $X \in \mathbb{R}^{(n_1+n_2) \times d}$ which is composed of $n_1$ unlabelled examples that an algorithm can actively query, and $n_2$ examples labelled a-priori. Concretely, denoting the true labels by $Y \in \mathbb{R}^{n_1 + n_2}$, the learner's objective is to find $\widehat{\beta} \in \mathbb{R}^d$ such that, \begin{equation} \| X \widehat{\beta} - Y \|_2^2 \le (1 + \epsilon) \min_{\beta \in \mathbb{R}^d} \| X \beta - Y \|_2^2 \end{equation} while making as few additional label queries as possible. In order to bound the label queries, we introduce an instance dependent parameter called the reduced rank, denoted by $R_X$, and propose an efficient algorithm with query complexity $O(R_X/\epsilon)$. This result directly implies improved upper bounds for two important special cases: (i) active ridge regression, and (ii) active kernel ridge regression, where the reduced-rank equates to the statistical dimension, $sd_\lambda$ and effective dimension, $d_\lambda$ of the problem respectively, where $\lambda \ge 0$ denotes the regularization parameter. For active ridge regression we also prove a matching lower bound of $O(sd_\lambda / \epsilon)$ on the query complexity of any algorithm. This subsumes prior work that only considered the unregularized case, i.e., $\lambda = 0$.

==> proof.tex <==
\newpage



\section{Active Linear regression with L2 regularization}

\textbf{Objective:}
Given a matrix $X \in \mathbb{R}^{n \times d}$ and $Y \in \mathbb{R}^n$.
To find $\widehat{\beta} \in \mathbb{R}^d$ such that,
\begin{equation}
    \| X \widehat{\beta} - Y \|_2^2 + \lambda \| \widehat{\beta} \|_2^2 \le (1 + \epsilon) \left( \min_{\beta \in \mathbb{R}^d} \| X \beta - Y \|_2^2 + \lambda \| \beta \|_2^2 \right)
\end{equation}
The learner is provided $X$ and the objective is to query as few $y$-labels as possible to find such a $\widehat{\beta}$.


% Let $\mathcal{F}$ be a family of linear functions from $\mathbb{R}^d \to \mathbb{R}$. %Let $\mathrm{v}_1,\mathrm{v}_2,\cdots,\mathrm{v}_d$ be a fixed orthonormal basis of $\mathcal{F}$ under $D$.
Let $U \Sigma V^T$ be the singular value decomposition of $X$. Define $D$ to be the uniform distribution over the rows of $X$.

We present \Cref{alg:RBSS} in this section and show that it is an $\epsilon$-well-balanced sampling procedure, defined as follows.


\begin{definition}\label{def:eps-w-b} [\citet[Def 2.1]{chen2019active}]
Consider a randomized algorithm $\textsf{Alg} (X,\epsilon)$ that outputs a set of points $\{ x_1,\cdots, x_m \}$ and weights $\{ w_1,\cdots,w_m \}$ as follows: in each iteration $i = 1,\cdots,m$, the algorithm chooses a distribution $D_i$ over the columns of $X$ to sample $x_i \sim D_i$. \textsf{Alg} is said to be an \textbf{$\epsilon$-well-balanced sampling procedure} if it satisfies the following two properties with probability at least $3/4$,
\begin{enumerate}
    \item For every $h \in \mathcal{F}$,
    \begin{align*}
        \sum_{i=1}^m w_i \langle h , x_i \rangle^2 \in \left[\frac{3}{4},\frac{5}{4}\right] \mathbb{E}_{x \sim D} \left[ \langle h , x \rangle^2 \right]
    \end{align*}
    Equivalently, the matrix $A = \textsf{diag} ( \{ \sqrt{w_i} \}_{i=1}^m) U \in \mathbb{R}^{m \times d}$ has $\lambda(A^T A)\in [3/4,5/4]$.
    \item For each $i \in [m]$, define $\alpha_i = \frac{D_i (x_i)}{D(x_i)} w_i$. Then, \textsf{Alg} must satisfy $\sum_{i=1}^m \alpha_i = O(1)$ and $\alpha_i K_{D_i} = O(\epsilon)$, where $K_{D_i}$ is the re-weighted condition number:
    \begin{align*}
        K_{D_i} = \sup_x \left\{ \sup_{h\in\mathcal{F}} \left\{ \frac{D_i(x)}{D(x)} \cdot\frac{\langle h , x \rangle^2}{\mathbb{E}_{x' \sim D} \left[ \langle h , x' \rangle^2 \right]} \right\} \right\} 
    \end{align*}
\end{enumerate}
\end{definition}

Define $\mathcal{E}$ as the event that the $\epsilon$-well-balanced sampling procedure \textsf{Alg} satisfies both conditions in \Cref{def:eps-w-b}. Note that $\mathrm{Pr} (\mathcal{E}) \ge 3/4$.

%Let $\mathrm{v}(x_i) = \left(\mathrm{v}_1(x_i), \mathrm{v}_2(x_i), \cdots, \mathrm{v}_d(x_i)\right)$. Let $X=U\Sigma V^T$ be the data matrix. Let $v_i$ be the $i^{th}$ row in $U$. Then $\mathrm{v}(x_i)$ would be $\sqrt{n}v_i$.

% The algorithm we consider was proposed by Chen and Price. We run the algorithm in this setting by augmenting the $n$ points with a set of $d$ points at the locations $\sqrt{\lambda} e_i$ with the labels $0$.

% We run Chen and Price's algorithm on this instance. The algorithm can be described as follows:

\begin{algorithm}[htb]
	\caption{\textsc{Chen+Price}}
	\label{alg:main}
	\begin{algorithmic}[1]
	    \State \textbf{Input:} $X \in \mathbb{R}^{n \times d}$; $Y \in \mathbb{R}^n$; accuracy parameter $\epsilon$; well balanced sampling procedure \textsf{Alg}.
		\State Repeat $\textsf{Alg} (X,\epsilon)$ until $\mathcal{E}$ is satisfied and let $ \{ x_1,\cdots, x_m \}$ and $\{ w_1,\cdots,w_m \}$ be the resulting set of points.
		\State Query the labels of $\{ x_1,\cdots, x_m \}$.
		\State \textbf{Return:} $\widehat{\beta} \gets \arg\min_{\beta \in \mathbb{R}^d} \sum_{i=1}^m w_i ( \beta^T x_i - y_i)^2 + \lambda \| \beta \|_2^2$.
	\end{algorithmic}
\end{algorithm}

The algorithm uses the $\epsilon$-well balanced sampling procedure to outputs weights and simply returns $\widehat{\beta}$ as the solution to the weighted ERM problem defined by $\{ x_1,\cdots, x_m \}$ and $\{ w_1,\cdots, w_m \}$.

\begin{lemma}
This lemma is to show that \cref{alg:main} works.
\end{lemma}

We consider the $\epsilon$-well balanced sampling procedure induced by the Randomized BSS algorithm proposed in \cite{lee2015constructing}.
Define $U(x)$ as the row in $U$ corresponding to $x$.

\begin{algorithm}[htb]
	\caption{\textsc{RandomizedBSS}}
	\label{alg:RBSS}
	\begin{algorithmic}[1]
	    \State \textbf{Input:} $X \in \mathbb{R}^{n \times d}$.
		\State \textbf{Initialization:} $j=0$; $\gamma = \sqrt{\epsilon}/C_0$; $u_0=2d/\gamma$; $l_0=-2d/\gamma$; $A_0 = 0$.
		\While{$(u_j-l_j)+\sum_{i = 0}^{j-1} \Phi_i^{\mathrm{Id}} < 8d/\gamma$}
		\State Define $\Phi_{j}^{\mathrm{Id}} = \textsf{Tr} \left( (u_j I - A_j)^{-1} (A_j - l_j I)^{-1} \right)$.
		\State Set coefficient $\alpha_j' = \frac{\gamma}{\Phi_{j}^{\mathrm{Id}}}$
		\State Sample a point $x$ with probability $p_x \triangleq \frac{U(x)^T \left( (u_j I - A_j)^{-1} + (A_j-l_jI)^{-1} \right) U(x)}{\Phi_j^{\mathrm{Id}}}$. Define the sampled point $x$ as $x_j$ and $p_x$ as $p_j$.
		\State Update $A_{j+1} \gets A_j + \frac{\gamma}{\Phi_{j}^{\mathrm{Id}}} \frac{1}{p_j} U(x_j) U(x_j)^T$
		\State Define the scaling factor $w_j' \gets \frac{\gamma}{\Phi_{j}^{\mathrm{Id}}} \frac{1}{p_j}$
		\State Update $u_{j+1} \gets u_j + \frac{\gamma}{1-2\gamma} \frac{1}{\Phi_{j}^{\mathrm{Id}}}$ and $l_{j+1} \gets l_j + \frac{\gamma}{1+2\gamma} \frac{1}{\Phi_{j}^{\mathrm{Id}}}$.
		\State $j \gets j+1$
		\EndWhile
		\State Assign $m=j$,
		\State Define $\midd \triangleq \frac{u_m+l_m}{2}$,
		\State Set coefficient $\alpha_j = \frac{\alpha_j'}{\midd}$ and the weight $w_j = \frac{w_j'}{\midd}$ for each $x_j$.
	    \State \textbf{Return} $\{ x_1,\cdots,x_m \}$; $\{ w_1,\cdots, w_m \}$; $A_m$.
	\end{algorithmic}
\end{algorithm}

\subsection*{Definitions}

For any PSD matrix $M$, define the potential function $\Phi_j^{M} = \textsf{Tr} ( M (u_j I - A_j)^{-1} + M (A_j - l_j I)^{-1}))$.

Define $\mathcal{F}_t$ as the filtration $\sigma ( \{x_1, \cdots, x_t\} )$ which encodes all the outcomes of the coin flips of the algorithm till the $t^{th}$ iteration.

\begin{lemma} \label{lemma:iterations}
Recall that \Cref{alg:RBSS} operates on $n+d$ points. The expected number of iterations the algorithm samples a point among the first $n$ is given by: $\mathbb{E} \left[ \sum_{j=1}^{m-1} \frac{\Phi_j^D}{\Phi_j^{\mathrm{Id}}} \right]$ where $D = \textsf{diag} \left( \left\{ \frac{1}{1 + \lambda / \sigma_i^2} \right\}_{i=1}^d \right)$.
\end{lemma}

\devvrit{Prove this}

\begin{lemma} \label{lemma:bounded}
For $\gamma < 1$, in each iteration $j = 0,\cdots,m$ of \Cref{alg:RBSS}, the condition $l_j I \preceq A_j \preceq u_j I$ is satisfied.
\end{lemma}
\begin{proof}
The proof follows by induction. For $j = 0$, $A_j = 0$ and trivially satisfies the condition $\frac{2d}{\gamma} I = -l_j I \preceq A_j \preceq u_j I = \frac{2d}{\gamma} I$. By the induction hypothesis, we assume that $l_j I \preceq A_j \preceq u_j I$ henceforth in the proof.  For any point $x$, observe that,
\begin{align}
    p_x \Phi_j^{\text{Id}} &= U(x)^T \left( (u_j I - A_j)^{-1} + (A_j - l_j I)^{-1} \right) U(x) \label{eq:1230}\\
    &\ge U(x)^T (u_j I - A_j)^{-1} U(x) \label{eq:1231}
\end{align}
Observe that for any vector $v$ and PSD matrix $B$, $vv^T \preceq (v^T B^{-1} v) B$.
Therefore, for any point $x$,
\begin{align}
    U(x) U(x)^T &\preceq (U(x)^T (u_j I - A_j)^{-1} U(x) ) (u_j I - A_j) \\
    &\overset{(i)}{\preceq} p_x \Phi_j^{\text{Id}} (u_j I - A_j) \label{eq:1232}
\end{align}
where $(i)$ uses \cref{eq:1231}.
Similarly by lower-bounding \cref{eq:1230} by $U(x)^T (A_j - l_j I)^{-1} U(x)$ and use a similar approach to prove that for any $x$,
\begin{equation} \label{eq:lA-lb}
    U(x) U(x)^T \preceq p_x \Phi_j^{\text{Id}} (A_j  - l_j I)
\end{equation}
Choosing $x = x_j$ in \cref{eq:1232}, as a special case, 
\begin{equation}
    A_{j+1} - A_j = \frac{\gamma}{p_j \Phi_j^{\text{Id}}} U(x_j) U(x_j)^T \preceq \gamma (u_j I - A_j) \label{eq:uA-ub}
\end{equation}
Using the induction hypothesis, we use this to prove that $A_{j+1} \preceq u_{j+1} I$. Indeed, \cref{eq:uA-ub} implies that,
\begin{equation}
(u_j I - A_j) - (u_j I - A_{j+1}) = A_{j+1} - A_j \preceq \gamma (u_j I - A_j)
\end{equation}
Therefore,
\begin{equation}
    (1-\gamma) (u_j I - A_j ) \preceq u_j I - A_{j+1} \preceq u_{j+1} I - A_{j+1}
\end{equation}
And using the induction hypothesis that $u_j I - A_j \succeq 0$ completes the proof that $A_{j+1} \preceq u_{j+1} I$. On the other hand, to prove that $A_{j+1} \succeq l_{j+1} I$, summing \cref{eq:lA-lb} over all $x$ and noting that $\sum_x U(x) U(x)^T = I$,
\begin{equation} \label{eq:1234}
    \frac{1}{\Phi_j^{\text{Id}}} I \preceq A_j - l_j I
\end{equation}
Finally, observe that,
\begin{align}
    A_{j+1} - l_{j+1} I &= (A_j - l_j I) + \left( \frac{\gamma}{\Phi_j^{\text{Id}}} \frac{1}{p_j} U(x_j) U(x_j)^T - \frac{\gamma}{1+2\gamma} \frac{1}{\Phi_j^{\text{Id}}} I \right) \\
    &\succeq (A_j - l_j I) - \frac{\gamma}{1+2\gamma} \frac{1}{\Phi_j^{\text{Id}}} I \\
    &\overset{(i)}{\succeq} \frac{1}{\Phi_j^{\text{Id}}} I - \frac{\gamma}{1+2\gamma} \frac{1}{\Phi_j^{\text{Id}}} I \\
    &\succeq 0
\end{align}
where $(i)$ uses \cref{eq:1234}. 
\end{proof}


\begin{lemma} \label{lemma:Phi-lb}
With probability $1$, in every iteration $0 \le j < m$ of the Chen and Price algorithm, $\Phi_j^{\mathrm{Id}} \ge \frac{1}{2} \gamma$.
\end{lemma}
\begin{proof}
Note that for $j \in [m-1]$, $\Phi_j^{\mathrm{Id}} = \textsf{Tr} ((u_j I - A_j)^{-1} + (A_j - l_j I)^{-1})$. Note that $A_j$ is a symmetric matrix. Suppose it is diagonalized as $U \Theta U^T$ where $\Theta = \textsf{diag} (\theta_1,\cdots,\theta_d)$ are its eigenvalues. Then, $\Phi_j^{\mathrm{Id}} = \sum_{t=1}^d \frac{1}{u_j - \theta_t} + \frac{1}{\theta_t - l_j}$. Lemma 5.3 in Chen+Price shows that $l_j I \preceq A_j \preceq u_j I$. With this constraint on the $\theta_t$'s, by minimizing, we obtain: $\frac{1}{u_j - \theta_t} + \frac{1}{\theta_t - l_j} \ge \frac{4}{u_j-l_j}$. Therefore, $\Phi_j^{\mathrm{Id}} \ge \frac{4d}{u_j - l_j}$. Furthermore, by the stopping criterion of the algorithm, in every iteration $j < m$ of the algorithm, $u_j - l_j \le \frac{8d}{\gamma}$. Therefore, for every $j = 0,1,\cdots,m-1$, $\Phi_j^{\mathrm{Id}} \ge \frac{1}{2} \gamma$.
\end{proof}


\begin{lemma} \label{lemma:umlm-ub}
For $\gamma < 1$, $u_m - l_m \leq 9d/\gamma$.
\end{lemma}
\begin{proof}
From \Cref{lemma:Phi-lb}, we know $\phi_{m-1}^{\mathrm{Id}} \geq \gamma/2$. Which implies $\gamma/\phi_{m-1}^{\mathrm{Id}} \leq 2$. By the stopping criterion of the algorithm, $u_{m-1} - l_{m-1} < 8d/\gamma$. Using these two,
\begin{align*}
    u_m-l_m &= u_{m-1}-l_{m-1} + \frac{\gamma}{\phi_{m-1}^{\mathrm{Id}}}\left(\frac{1}{1-2\gamma} - \frac{1}{1+2\gamma}\right)\\
    &\leq 8d/\gamma + 2\left(\frac{1}{1-2\gamma} - \frac{1}{1+2\gamma}\right)\\
    &\leq 9d/\gamma
\end{align*}
\end{proof}

% \begin{lemma} \label{lemma:Phim-lb}
% With probability $1$, $\Phi_m^{\mathrm{Id}} \ge \frac{4}{9} \gamma$.
% \end{lemma}
% \begin{proof}
% The proof follows from \Cref{lemma:umlm-ub} and using a similar argument as in the proof of \Cref{lemma:Phi-lb}.
% \end{proof}

% \devvrit{Correct things below}
A conclusion from \Cref{lemma:iterations,lemma:Phi-lb} is that the expected number of points among the first $n$ sampled by the algorithm is $\le \mathbb{E} \left[ \frac{2}{\gamma} \sum_{j=1}^{m-1} \Phi_j^D \right]$.

Note that the event $\{ m > j \} = \left\{ u_j - l_j + \sum_{i=0}^{j-1} \Phi_i^{\text{Id}} < \frac{8d}{\gamma} \right\}$ is measurable with respect to $\mathcal{F}_{j-1}$ (so it is a stopping time). Likewise, the random variable $\Phi_j^D$ is measurable with respect to $\mathcal{F}_{j-1}$. Therefore, by Wald's equation,
\begin{equation}
    \mathbb{E} \left[ \# \text{ sampled} \right] \le \frac{2}{\gamma} \mathbb{E} \left[ \sum_{j=0}^{m-1} \Phi_j^D \right] \le \frac{2}{\gamma} \mathbb{E} \left[ \sum_{j=0}^{m-1} \mathbb{E} \left[ \Phi_j^D \right] \right].
\end{equation}
\devvrit{make this equation better notation wise}

\begin{lemma} \label{lemma:Phi-ub}
For any fixed PSD matrix $M$, $\mathbb{E} [\Phi_{j+1}^M] \le \mathbb{E} [\Phi_{j}^M ]$. 
\end{lemma}
\begin{proof}
Recall that $\Phi_j^M = \textsf{Tr} ( M(u_j I - A_j)^{-1} + \textsf{Tr} ( M(A_j - l_j I)^{-1})$. $\Phi^M_{j+1}$ can be written as $\textsf{Tr} ( M(u_{j+1} I - A_j - w_j w_j^T)^{-1)} + \textsf{Tr} ( M (A_j + w_j w_j^T - l_{j+1} I)^{-1})$. Following a similar approach as BSS Lemma 3.3 and 3.4, invoking the Sherman-Morrison inversion formula,
\begin{equation}
    \left(u_{j+1} I - A_j - w_j w_j^T \right)^{-1} = (u_{j+1} I - A_j)^{-1} + \frac{(u_{j+1} I - A_j)^{-1} w_j w_j^T (u_{j+1} I - A_j)^{-1}}{1 - w_j^T (u_{j+1} I - A_j)^{-1} w_j}.
\end{equation}
Multiplying by $M$ and tracing both sides,
\begin{equation}
   \textsf{Tr} \left(M \left(u_{j+1} I - A_j - w_j w_j^T \right)^{-1} \right) = \textsf{Tr} (M (u_{j+1} I - A_j)^{-1}) + \frac{\textsf{Tr} (M (u_{j+1} I - A_j)^{-1} w_j w_j^T (u_{j+1} I - A_j)^{-1})}{1 - w_j^T (u_{j+1} I - A_j)^{-1} w_j}.
\end{equation}
Note that with probability $1$, $w_j w_j^T \preceq \gamma (u_j I - A_j) \preceq \gamma (u_{j+1} I - A_j)$. Therefore, $w_j^T (u_{j+1} - A_j)^{-1} w_j \le \gamma$. Therefore,
\begin{equation}
    \textsf{Tr} \left(M\left(u_{j+1} I - A_j - w_j w_j^T \right)^{-1} \right) \le \textsf{Tr} (M(u_{j+1} I - A_j)^{-1}) + \frac{\textsf{Tr} (M(u_{j+1} I - A_j)^{-1} w_j w_j^T (u_{j+1} I - A_j)^{-1})}{1 - \gamma}.
\end{equation}
Finally, using linearity of expectation and noting that $\mathbb{E} \left[w_j w_j^T \middle| A_j \right] = \frac{\gamma}{\Phi_j^{\mathrm{Id}}} I$, we have that,
\begin{align}
    \mathbb{E} \left[ \textsf{Tr} \left( M\left(u_{j+1} I - A_j - w_j w_j^T \right)^{-1} \right) \right] &\le \mathbb{E} \left[ \textsf{Tr} (M(u_{j+1} I - A_j)^{-1}) \right] + \mathbb{E} \left[ \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1 - \gamma)} \textsf{Tr} (M(u_{j+1} I - A_j)^{-2}) \right]. \label{eq:13}
\end{align}
By a similar calculation as before,
\begin{align} \label{eq:14}
    \mathbb{E} \left[ \textsf{Tr} \left(M\left(A_j + w_j w_j^T - l_{j+1} I  \right)^{-1} \right) \right] &\le \mathbb{E} \left[ \textsf{Tr} (M(A_j - l_{j+1} I )^{-1}) \right] - \mathbb{E} \left[ \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1+2\gamma)} \textsf{Tr} \left(M(A_j - l_{j+1} I )^{-2} \right) \right].
\end{align}
Note the difference from before, for $\gamma \le \frac{1}{4}$, we use the inequality $w_j w_j^T \preceq 2\gamma (A_j - l_{j+1} I)$ which we derive in \Cref{lemma:wjwjT-l}. This appears as the $1+2\gamma$ factor in the denominator of the second term in \cref{eq:14}.

Now observe that, $u_{j+1} - u_j = \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1-2\gamma)} \ge \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1-\gamma)}$ and $l_{j+1} - l_j = \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1+2\gamma)}$. Therefore, adding \cref{eq:13} and \cref{eq:14} together,
\begin{align}
    \mathbb{E} \left[ \Phi^M_j \right] \le& \mathbb{E} \left[ \textsf{Tr} (M(u_{j+1} I - A_j )^{-1} + M(A_j - l_{j+1} I )^{-1}) \right] \nonumber\\
    &+ \mathbb{E} \left[ (u_{j+1} - u_j) \textsf{Tr} (M(u_{j+1} I - A_j)^{-2}) - (l_{j+1} - l_j) \textsf{Tr} (M(A_j - l_{j+1} I)^{-2}) \right] \label{eq:16}
\end{align}
Define $\Delta_u = u_{j+1} - u_j$ and $\Delta_l = l_{l+1} - l_j$ and for $t \in [0,1]$, define the function
\begin{equation}
    f (t) = \textsf{Tr} \Big( M( (u_j + \Delta_u t) I - A_j)^{-1} + M(A_j - (l_j + t \Delta_l) I)^{-1} \Big).
\end{equation}
 Under the assumption $l_j I \preceq A_j \preceq u_j I$, the function $f(t)$ is convex in $t$. Therefore, $f(0) - f(1) \ge - \frac{\mathrm{d} f(t)}{\mathrm{d}t} \Big|_{t=1}$. In \cref{eq:16} observe that the RHS is precisely $f(1) - \frac{\mathrm{d} f(t)}{\mathrm{d}t} \Big|_{t=1}$. Upper bounding this by $f(0)$, results in the equation
 \begin{equation}
     \mathbb{E} [\Phi_{j+1}^M] \le \mathbb{E} \left[ \textsf{Tr} (M(u_j I - A_j )^{-1} + M(A_j - l_j I )^{-1}) \right] = \mathbb{E} [\Phi_j^M].
 \end{equation}
\end{proof}

\begin{lemma} \label{lemma:wjwjT-l}
For $\gamma \le \frac{1}{4}$, $w_j w_j^T \preceq 2\gamma (A_j - l_{j+1} I)$.
\end{lemma}
\begin{proof}
First observe that,
\begin{equation} \label{eq:15}
    w_j w_j^T \preceq \gamma (A_j - l_j I) = \gamma (A_j - l_{j+1} I) + \gamma (l_{j+1} - l_j) I
\end{equation}
Therefore, it suffices to show that $l_{j+1} - l_j \preceq (A_j - l_{j+1} I)$, or in other words, $l_{j+1} - l_j \le \lambda_{\min} (A_j - l_{j+1} I)$ to complete the proof. By definition,
\begin{align}
    l_{j+1} - l_j = \frac{\gamma}{(1-2\gamma)\Phi_j^{\mathrm{Id}}} \le \frac{\gamma}{1-2\gamma} \lambda_{\min} (A_j - l_j I) \le \frac{1}{2} \lambda_{\min} (A_j - l_j I)
\end{align}
where the last inequality uses the fact that $\gamma \le \frac{1}{4}$. Therefore, $2 l_{j+1} - l_j \le \lambda_{\min} (A_j)$ and $l_{j+1} - l_j \le \lambda_{\min} (A_j - l_{j+1})$. Plugging this back into \cref{eq:15},  we arrive at the claim of the lemma.
\end{proof}

\begin{corollary}
For any fixed PSD matrix, $M$, $\mathbb{E} [ \sum_{j=0}^{m-1} \Phi_j^M] \le \left(\frac{1}{u_0} - \frac{1}{l_0} \right) \mathbb{E} [m] \textsf{Tr} (M)$. In particular,
\begin{enumerate}
    \item[(i)] $\mathbb{E} [ \sum_{j=0}^{m-1} \Phi_j^{\mathrm{Id}}] \le \left(\frac{1}{u_0} - \frac{1}{l_0} \right) \mathbb{E} [m] d$;
    \item[(ii)] $\mathbb{E} [ \sum_{j=0}^{m-1} \Phi_j^D] \le \left(\frac{1}{u_0} - \frac{1}{l_0} \right) \mathbb{E} [m] \textsf{sd}_\lambda$.
\end{enumerate}
\end{corollary}
\begin{proof}
From Wald's equation,
\begin{align}
    \mathbb{E} \left[ \sum_{j=0}^{m-1} \Phi_j^M \right] &= \mathbb{E} \left[ \sum_{j=0}^{m-1} \mathbb{E} \left[ \Phi_j^M \right] \right] \\
    &\overset{(i)}{\le} \mathbb{E} \left[ \sum_{j=0}^{m-1} \mathbb{E} \left[ \Phi_0^M \right] \right] \\
    &= \mathbb{E} \left[ m \right] \mathbb{E} \left[ \Phi_0^M \right] \\
    &= \mathbb{E} \left[ m \right] \textsf{Tr} (M (u_0I)^{-1} + M (-l_0 I)^{-1}) \\
    &= \left(\frac{1}{u_0} - \frac{1}{l_0} \right) \mathbb{E} [m] \textsf{Tr} (M)
\end{align}
where $(i)$ follows from \Cref{lemma:Phi-ub}.
\end{proof}

Since $u_0 = \frac{2d}{\gamma}$ and $l_0 = -\frac{2d}{\gamma}$,
\begin{equation}
    \# \text{ sampled} \le \frac{2}{\gamma} \mathbb{E} \left[ \sum_{j=0}^{m-1} \Phi_j^D \right] \le \frac{2}{\gamma} \left( \frac{1}{u_0} - \frac{1}{l_0} \right) \mathbb{E} [m] \textsf{Tr} (D) \le \frac{2}{d} \textsf{sd}_\lambda \mathbb{E} [m]
\end{equation}

\begin{lemma}
With probability $1$, $m \le \frac{2d}{\gamma^2}$.
\end{lemma}
\begin{proof}
% In every iteration before the algorithm terminates, from \Cref{lemma:Phi-lb}, $\Phi_j^{\mathrm{Id}} \ge \frac{1}{4} \gamma$.
Assuming that the algorithm has not terminated till the $(t+1)^{th}$ iteration, $u_t - l_t = u_0 - l_0 + \sum_{j=0}^{t-1} \frac{4\gamma^2}{\Phi_j^{\mathrm{Id}} (1-4\gamma^2)} < \frac{8d}{\gamma}$ (this uses the fact that $u_{j+1} - u_j = \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1-2\gamma)}$ and $l_{j+1} - l_j = \frac{\gamma}{\Phi_j^{\mathrm{Id}} (1+2\gamma)}$). Observe that the event,
\begin{align}
    \{ m \ge t \} &= \{ u_t - l_t < 8d/\gamma \} \overset{(i)}{=} \left\{ \sum_{j=0}^{t-1} \frac{4\gamma^2}{\Phi_j(1-4\gamma^2)} + \sum_{j=0}^{t-1}\Phi_j^{\mathrm{Id}} < \frac{4d}{\gamma} \right\} \overset{(ii)}{\subseteq} \left\{ 2\gamma \cdot t < \frac{4d}{\gamma} \right\}
\end{align}
% &\overset{(ii)}{\le} \mathrm{Pr} \left( \frac{8d (1-4\epsilon^2) t^2}{4\epsilon^3} < \sum_{j=0}^{t-1} \Phi_j \right)
where $(i)$ uses the fact that $u_{j+1} - l_{j+1} = u_j - l_j + \frac{\gamma}{\Phi_{j} (1-2\gamma)} - \frac{\gamma}{\Phi_{j} (1+2\gamma)}$ with $u_0 - l_0 = \frac{4d}{\gamma}$, and the  $(ii)$ uses the AM$\ge$GM inequality. Therefore, with $t = \frac{2d}{\gamma^2}$, the event $\{ m \ge t \}$ happens with probability $0$.
\end{proof}
% $(ii)$ uses the fact that $\left( \sum_{j=0}^{t-1} \frac{1}{\Phi_j} \right) \left( \sum_{j=0}^{t-1} \Phi_j \right) \ge t^2$.
% Integrating both sides from $t = 0$ to $t = \infty$ and noting the fact that for a non-negative random variable $X$, $\mathbb{E} [X] = \int_{t = 0}^\infty \mathrm{Pr} (X \ge t) \mathrm{d}t$. We get that,
% \begin{equation}
%     \mathbb{E} [m] \le \sqrt{\frac{4 \epsilon^3}{8d (1-4\epsilon^2)}} \mathbb{E} \left[ \sqrt{\sum_{j=0}^{t-1} \Phi_j} \right] \overset{(i)}{\le} \sqrt{\frac{4 \epsilon^3}{8d (1-4\epsilon^2)}} \sqrt{\mathbb{E} \left[ \sum_{j=0}^{t-1} \Phi_j \right]}.
% \end{equation}
% where $(i)$ uses Jensen's inequality and the concavity of $\sqrt{\cdot}$.


\begin{lemma} \label{lemma:um-lb}
For $\gamma < \frac{1}{4}$, with probability at least $1-p$, $u_m \geq \frac{p^2d}{8\gamma^2}$.
\end{lemma}
\begin{proof}
First, observe that $u_m > \sum_{j=0}^{m-1}\frac{\gamma}{\Phi_j^{\mathrm{Id}}}$ and $\left( \sum_{j=0}^{t-1} \frac{1}{\Phi_j} \right) \left( \sum_{j=0}^{t-1} \Phi_j \right) \ge t^2$, we want to analyze
\begin{align}
    \mathrm{Pr}\left( \frac{p^2 d}{8 \gamma^3} \leq \frac{m^2}{\sum_{j=0}^{m-1} \Phi_j^{\mathrm{Id}}}\right) &= \mathrm{Pr}\left(\sum_{j=0}^{m-1} \Phi_j^{\mathrm{Id}} \cdot \frac{p^2 d}{8 \gamma^3} \leq m^2\right)\\
    &\overset{(i)}\geq \mathrm{Pr}\left(\frac{p^2 d^2}{\gamma^4} \leq m^2\right)
\end{align}
Where the last sufficient condition $(i)$ comes from the stopping criterion, which implies $\sum_{j=0}^{m-1} \Phi_j^{\mathrm{Id}} \leq \frac{8d}{\gamma}$.

\noindent Now we prove an upper bound to $\mathrm{Pr}(m < g)$ where $g \triangleq \frac{pd}{\gamma^2}$.
\begin{align*}
    \mathrm{Pr}\left(m < g \right) &\overset{(i)}= \mathrm{Pr}\left( \sum_{j=0}^{g-1} \frac{\gamma^2}{\Phi_j^{\mathrm{Id}} (1 - 4\gamma^2)} + \frac{4d}{\gamma} + \sum_{j=0}^{g-1} \Phi_j^{\mathrm{Id}} \geq \frac{8d}{\gamma}  \right)\\
    &\overset{(ii)}\leq \frac{\mathbb{E}\left[\sum_{j=0}^{g-1}\frac{\gamma^2}{\Phi_j^{\mathrm{Id}} (1 - 4\gamma^2)} + \sum_{j=0}^{g-1} \Phi_j^{\mathrm{Id}}\right]}{4d/\gamma}\\
    &\overset{(iii)}\leq \frac{g\mathbb{E}[\Phi_0^{\mathrm{Id}}] + \frac{\gamma^2}{1 - 4\gamma^2} \mathbb{E}\left[ \sum_{j=0}^{g-1}\frac{1}{\Phi_j^{\mathrm{Id}}} \right]}{4d/\gamma}\\
    &\overset{(iv)}\leq \frac{g\gamma + \frac{2 \gamma g}{1 - 4\gamma^2}}{4d/\gamma}
\end{align*}
where $(i)$ comes form the stopping criterion and the update rules for $u_j$ and $l_j$, $(ii)$ is Markov's inequality, $(iii)$ follows by \Cref{lemma:Phi-ub}, and $(iv)$ from \Cref{lemma:Phi-lb}. Using the fact that $\gamma < \frac{1}{4}$,
\begin{align}
    \mathrm{Pr}\left(m < g \right) &\le \frac{g\gamma^2}{d} = p
\end{align}
\end{proof}


Define the event $\Gamma$ as the event that $\{ u_m \ge \frac{d}{64\gamma^2}\}$. From \Cref{lemma:um-lb}, $\mathrm{Pr} (\Gamma) \ge \frac{3}{4}$.

\begin{lemma}
For $\gamma \leq \frac{1}{300}$, if the event $\Gamma$ occurs, $l_m > 0$.
\end{lemma}
\begin{proof}
First observe that,
\begin{align}
    u_m &= u_0 + \frac{\gamma}{(1-2\gamma)}\sum_{j=0}^{m-1}\frac{1}{\Phi_j^{\mathrm{Id}}}\\
    \implies &\sum_{j=0}^{m-1}\frac{1}{\Phi_j^{\mathrm{Id}}} = \left(u_m-\frac{2d}{\gamma}\right) \left( \frac{1-2\gamma}{\gamma} \right)\\
    \implies &l_m = \frac{-2d}{\gamma} + \frac{\gamma}{1+2\gamma} \left(u_m-\frac{2d}{\gamma}\right) \left( \frac{1-2\gamma}{\gamma} \right)
\end{align}
Thus if $u_m$ is large enough, the RHS will be $> 0$. It suffices to assume $\gamma
\leq \frac{1}{300}$ for this statement to be true since conditioned on $\Gamma$, $u_m \ge \frac{d}{64 \gamma^2}$.
\end{proof}

\begin{lemma} \label{lemma:3456}
Conditioned on the event $\Gamma$, Algorithm \ref{alg:RBSS} returns matrix $A_m$ with condition number $\frac{\lambda_{\max} (A_m)}{\lambda_{\min} (A_m)} \le \frac{u_m}{l_m} \le 1+3456\gamma$, for $\gamma \leq \frac{1}{7 00}$.
\end{lemma}
\begin{proof}
From \Cref{lemma:bounded}, the condition number of $A_m$ is at most,
\begin{align}
    \frac{u_m}{l_m} = \left(1 - \frac{u_m-l_m}{u_m}\right)^{-1}
\end{align}
Hence, it suffices to prove that conditioned on the event $\Gamma$, $(u_m-l_m)/u_m$ is $\leq c\gamma$, assuming that $c\gamma\leq \frac{5}{6}$. We know from \Cref{lemma:umlm-ub}, $u_m-l_m \leq  \frac{9d}{\gamma}$. Hence, it suffices to show that under the event $\Gamma$,
\begin{align}
    \frac{9d/\gamma}{u_k} \leq c\gamma
    \iff \frac{9d}{c\gamma^2} \leq u_m
\end{align}
Conditioned on the event $\Gamma$, $u_m \ge \frac{d}{64\gamma^2}$. Therefore, it suffices to choose $c \ge 576$. As $\gamma \leq \frac{1}{700}, c\gamma \leq \frac{5}{6}$. Finally,
\begin{equation}
    \left(1 - \frac{u_m-l_m}{u_m}\right)^{-1} \le 1 + \frac{c \gamma}{1 - c \gamma} \le 1 + 3456 \gamma.
\end{equation}

\end{proof}

\devvrit{mention that $A$ is defined as $\frac{A_m}{\midd}$}

\begin{lemma}\label{lem:AstartA}
Conditioned on $\Gamma$, $(1 - 1728 \gamma) I \preceq A^T A \preceq (1 + 1728 \gamma) I$.
\end{lemma}
\begin{proof}
From \Cref{lemma:3456}, $\frac{u_m}{l_m} \le 1 + 3456 \gamma$.
\begin{align*}
    A^T A = \frac{1}{\midd}\sum_{j=1}^{m} w'_j U (x_j) U(x_j)^T = \frac{A_m}{\midd}
\end{align*}
Therefore, $\lambda(A^T A) \in \left[\frac{l_m}{\midd},\frac{u_m}{\midd}\right]$. Also, given $\frac{u_m}{l_m} \leq 1 + 3456\gamma$, we have
\begin{align}
    \frac{u_m+l_m}{l_m} &\leq 2+3456\gamma\\
    \implies \frac{2}{2 + 3456\gamma} &\leq \frac{l_m}{\frac{u_m+l_m}{2}} \\
    \implies 1 - 1728\gamma &\leq \frac{l_m}{\midd}
\end{align}
A similar approach can be used to prove that $\frac{u_m}{\midd} \leq 1 + 1728\gamma$.
\end{proof}

\begin{lemma}
\Cref{alg:RBSS} is an $\epsilon$-well-balanced sampling procedure.
\end{lemma}
\begin{proof}
To show that \Cref{alg:RBSS} is an $\epsilon$-well-balanced sampling procedure, recall from the definition that we must show that with probability $\ge \frac{3}{4}$,
\begin{enumerate}
    \item $\frac{3}{4} I \preceq A^T A \preceq \frac{5}{4} I$
    \item $\sum_{j=0}^{m-1} \alpha_j = O(1)$ and for all $j=0,\cdots,m-1$, $\alpha_j K_{D_j} = O(\epsilon)$.
\end{enumerate}
Conditioned on the event $\Gamma$ which holds with probability $\ge \frac{3}{4}$, we show that both of these properties hold. 

From \Cref{lem:AstartA}, with $\gamma \le \frac{1}{6912}$, conditioned on $\Gamma$, we have that $\frac{3}{4} I \preceq A^T A \preceq \frac{5}{4} I$ which shows that the first property is satisfied.

On the other hand, to bound $\sum_{j=0}^{m-1} \alpha_j$, observe that
\begin{align*}
    \sum_{j=0}^{m-1}\alpha_j &=  \sum_{j=0}^{m-1}\frac{\gamma}{\phi_j^{\mathrm{Id}}}\cdot    \frac{1}{\midd} \leq \sum_{j=0}^{m-1}\frac{4}{\frac{u_m+l_m}{2}} \leq \frac{2d}{\gamma^2}\frac{8}{u_m} \leq 1024
\end{align*}
where we use the fact that $u_m \ge \frac{d}{64 \gamma^2}$ conditioned on $\Gamma$. Following the proof of \citet[Lemma 5.1]{chen2019active}, we bound $\alpha_j K_{D_j}$ as follows:
\begin{align*}
    \alpha_jK_{D_j} = \frac{\gamma}{\midd}\cdot \frac{u_j-l_j}{2} = \gamma\frac{u_j-l_j}{u_m+l_m} \leq 512\gamma^2 = \frac{512 \epsilon}{C_0^2}
\end{align*}
where we upper bound $u_j-l_j \leq \frac{8d}{\gamma}$ using the stopping criterion of \Cref{alg:RBSS}, and lower bound $u_m+l_m\geq u_m \geq d/64\gamma^2$ conditioned on the event $\Gamma$. We also substitute $\gamma = \frac{\sqrt{\epsilon}}{C_0}$ and choose $C_0$ appropriately.
\end{proof}
